Online Continual Knowledge Learning for Language Models

Large Language Models (LLMs) serve as repositories of extensive world knowledge, enabling them to perform tasks such as question-answering and fact-checking. However, this knowledge can become obsolete as global contexts change. In this paper, we introduce a novel problem in the realm of continual learning: Online Continual Knowledge Learning (OCKL). This problem formulation aims to manage the dynamic nature of world knowledge in LMs under real-time constraints. We propose a new benchmark and evaluation metric designed to measure both the rate of new knowledge acquisition and the retention of previously learned knowledge. Our empirical evaluation, conducted using a variety of state-of-the-art methods, establishes robust base-lines for OCKL. Our results reveal that existing continual learning approaches are unfortunately insufficient for tackling the unique challenges posed by OCKL. We identify key factors that influence the trade-off between knowledge acquisition and retention, thereby advancing our understanding of how to train LMs in a continually evolving environment.

==> 1_abstract.tex <==
\begin{abstract}
% % ============ rewrite according to ICLR 22 toward =================
 % Large Language Models (LMs) have the ability to store extensive world knowledge in their parameters due to pretraining on a vast amount of web corpus. This knowledge can be leveraged to perform knowledge-dependent downstream tasks such as question-answering and open dialogue.
\begin{comment}
Language Models (LMs) can encapsulate a substantial amount of world knowledge within their parameters by being pre-trained on an extensive collection of corpus. This reservoir of knowledge can be utilized to effectively undertake knowledge-dependent tasks, including question-answering and fact-checking. In practical scenarios, the world knowledge stored in language models may become outdated as the world evolves, while training these models remains time-consuming. Hence, it is crucial to consider time constraints to maintain constantly evolving LMs, ensuring efficient acquisition of new knowledge and preventing catastrophic forgetting at the same time. To propel the continual learning community into more realistic scenarios, we introduce a novel continual learning (CL) problem namely \textit{Online Continual Knowledge Learning} (\textbf{\dataset}). We construct a new benchmark and metric for real-time evaluation to quantify the practical and efficient rate of knowledge acquisition and t he ability to retain previously acquired knowledge in LMs. We have employed a wide range of recent approaches from the literature to establish a set of strong baselines. Through extensive experiments, we discover that OCKL presents distinct challenges that have not been adequately addressed in any existing approaches. By elucidating the key factors affecting the balance between knowledge acquisition and forgetting, we demonstrate that OCKL represents a complex and significant challenge that enhances our comprehension of and ability to train LMs in real-time constraints continually. The benchmark datasets, evaluation script, and baseline code to reproduce our results will be made publicly available.     
\end{comment}
Large Language Models (LLMs) serve as repositories of extensive world knowledge, enabling them to perform tasks such as question-answering and fact-checking. However, this knowledge can become obsolete as global contexts change.
% , and updating these models is computationally expensive. To address this, 
In this paper, we introduce a novel problem in the realm of continual learning: \textit{Online Continual Knowledge Learning} (\textbf{OCKL}). This problem formulation aims to manage the dynamic nature of world knowledge in LMs under real-time constraints. We propose a new benchmark and evaluation metric designed to measure both the rate of new knowledge acquisition and the retention of previously learned knowledge. Our empirical evaluation, conducted using a variety of state-of-the-art methods, establishes robust baselines for OCKL. Our results reveal that existing continual learning approaches are unfortunately insufficient for tackling the unique challenges posed by OCKL. We identify key factors that influence the trade-off between knowledge acquisition and retention, thereby advancing our understanding of how to train LMs in a continually evolving environment.

% Language Models (LMs) can encapsulate a substantial amount of world knowledge within their parameters by being pre-trained on an extensive collection of corpus. This reservoir of knowledge can be utilized to undertake knowledge-dependent tasks, including question-answering and fact-checking effectively. However, the world knowledge stored in LMs may become outdated as global contexts evolve, and retraining these models is time-intensive. It is vital to incorporate time constraints into the sustained management of perpetually evolving LMs, thereby ensuring instruction responses to directives related to the latest global knowledge. Throughout this process, it is paramount to secure the efficient assimilation of new information while concurrently preventing catastrophic forgetting. To advance the continual learning community towards more realistic scenarios, we introduce a novel continual learning (CL) problem, termed \textit{Online Continual Knowledge Learning} (\textbf{OCKL}). We establish a new benchmark and metric for real-time evaluation to quantify the practical and efficient rate of knowledge acquisition and retention of previously acquired knowledge in LMs. Using a wide range of recent approaches from the literature, we establish a set of robust baselines. Through comprehensive experiments, we identify that OCKL poses unique challenges not adequately addressed by existing approaches. By highlighting the critical factors that influence the balance between knowledge acquisition and forgetting, we illustrate that OCKL presents a complex and significant challenge, enhancing our understanding and ability to train LMs under continuous, real-time constraints. 
% The benchmark datasets, evaluation script, and the baseline code to reproduce our results will be publicly available.

%=================================================================
% ACL vision
% Language models (LMs) have the capacity to encapsulate a substantial wealth of world knowledge within their parameters through pre-training on a vast corpus. This reservoir of knowledge can be effectively leveraged to perform knowledge-dependent tasks such as Q\&A and fact-checking. However, the world knowledge embedded in LMs may become obsolete as global contexts evolve, and retraining these models is a time-intensive process. It is crucial to incorporate time constraints into the ongoing management of perpetually evolving Large Language Models (LMs) to ensure instruct responses to directives related to the latest global knowledge. Throughout this process, it is of paramount importance to facilitate the efficient assimilation of new information while simultaneously guarding against catastrophic forgetting. We make multiple contributions to initiate research on this task. First, we introduced a novel streaming dataset \textit{Online Continual Knowledge Learning} (\textbf{\dataset}), which contains Knowledge stream and Q\&A stream. Second, we proposed metrics for learning speed and knowledge gap to evaluate various continual learning methods on \dataset. Through extensive experiments, we found that \dataset presents unique challenges not covered by existing approaches, emphasizing the critical factors affecting the balance between knowledge acquisition and forgetting. 

% Continual Learning (CL) research often assumes unrestricted training time for evaluations, a condition that is impractical, particularly for language models (LMs), where real-time adaptability is crucial. This paper highlights the importance of real-time evaluations for CL methods in the context of continuing pre-training of LMs, which is particularly pertinent given the dynamic nature of data streams.
% %
% In attempting to implement real-time evaluation, we encounter two key challenges: the scarcity of datasets that cover diverse time granularities and the complexity of effectively combining various CL components frequently found in the literature, such as core-set selection, memory sampling strategies, regularization methods, and parameter-expansion approaches.
% %
% In response, we conduct an exhaustive analysis of current CL methods for LMs, emphasizing computational efficiency. We carry out a series of extensive experiments using the \dataset dataset, which comprises 58 million time-stamped events (the ``knowledge stream'') and a corresponding question-answer test stream (the ``QA stream'').
% %
% Our findings indicate that all CL methods fall short in a real-time evaluation setting, largely due to the redundancy and subpar quality of the text stream data. To tackle these performance issues, we have begun exploring the core-set selection solution. Preliminary results show promising improvements, with performance gains of up to XXX in the XXXX.

% Current evaluations of Continual Learning (CL) methods typically assume that there is no constraint on training time and computation. This is an unrealistic assumption for any real-world setting, which motivates us to propose: a practical real-time evaluation of continual learning, in which the stream does not wait for the model to complete training before revealing the next data for predictions. To do this, we evaluate current CL methods with respect to their computational costs. We conduct extensive experiments on CLOC, a large-scale dataset containing 39 million time-stamped images with geolocation labels. We show that a simple baseline outperforms state-of-the-art CL methods under this evaluation, questioning the applicability of existing methods in realistic settings. In addition, we explore various CL components commonly used in the literature, including memory sampling strategies and regularization approaches. We find that all considered methods fail to be competitive against our simple baseline. This surprisingly suggests that the majority of existing CL literature is tailored to a specific class of streams that is not practical. We hope that the evaluation we provide will be the first step towards a paradigm shift to consider the computational cost in the development of online continual learning methods.

% % ============ rewrite according to Chunwei's suggestions =================
% Continual Learning (CL) research often assumes unrestricted training time, which is impractical for LMs when (near) real-time adaptability is required.
% %
% Despite a recent study on the practical real-time evaluation of continual learning, there are still two key challenges that remain to be solved in the context of LMs.
% First, the scarcity of text datasets that cover diverse time granularities; 
% Second, the complexity of effectively combining various CL components frequently found in the literature, such as core-set selection, memory sampling strategies, regularization methods, and parameter-expansion approaches.
% %
% This paper highlights the importance of real-time evaluations for CL methods in continuing pre-training of LMs, which is non-trivial given the dynamic nature of data streams.
% %
% We introduce a novel Online Continual Knowledge Learning (OCKL) benchmark designed for language model pre-training, by constructing a dynamic knowledge \dataset dataset including diverse time granularities that comprise over 90 thousand time-stamped events (i.e. ``Knowledge stream'') and a corresponding question-answer test stream (i.e. ``QA stream'').
% %
% Besides, we propose \textbf{Knowledge Gap} (KG) to measure the LMs’ capability of learning time-changing knowledge. 
% %
% We conduct extensive experiments on the continuous learning method with \dataset.
% %
% Our findings indicate that most CL methods fall short in a real-time evaluation setting, largely due to the transient exposure time and the subpar quality of the text stream data while \dataset prefers parameter-expansion methods for both accuracy and speed. 
% \cc{
% We have further evaluated a simple method that expedites the training process while maintaining an acceptable level of performance compared to state-of-the-art CL methods under this evaluation.
% } 
% %
% We hope that the evaluation we present serves as the initial stride towards ushering in a paradigm shift, encouraging the consideration of knowledge update efficiency in the development of online continual knowledge learning.
% % To tackle these performance issues, we have begun exploring the core-set selection solution. 
% % The preliminary results show promising improvements, with performance gains of up to 708(token/s).

\end{abstract}


==> 2-Introduction.tex <==
\section{Introduction}
Large Language Models like LLaMa2~\citep{touvron2023llama} and GPT-3~\citep{brown2020language} have demonstrated remarkable proficiency in Knowledge Intensive Language Tasks (KILT)~\citep{petroni2021kilt}. Despite their success, a significant limitation is their struggle to adapt to rapidly evolving global knowledge, as highlighted by their performance in the LAnguage Model Analysis (LAMA) framework~\citep{petroni2019language}. The conventional method of augmenting LLMs with an external, continually updated knowledge base introduces latency and reduces the models' capacity for real-time contextual understanding~\citep{raffel2019exploring}.

% Large Language Models (LLMs) such as LLaMa2~\citep{touvron2023llama} and GPT-3~\citep{brown2020language} have shown remarkable efficacy in Knowledge Intensive Language Tasks (KILT)~\citep{petroni2021kilt}. These models have been rigorously evaluated using the LAnguage Model Analysis (LAMA) framework~\citep{petroni2019language}, confirming their ability to encapsulate a wealth of world knowledge. However, they struggle to adapt to rapidly evolving global contexts. While one could consider augmenting LLMs with an external, continually updated knowledge base, this approach introduces latency and hampers the model's contextual understanding of new data~\citep{raffel2019exploring}.

\begin{figure}[t]
\includegraphics[width=0.45\textwidth]{fig/CL-LMs.pdf}
    \caption{\small Static models like T5~\citep{2020t5}, due to their knowledge cutoff, cannot provide timely answers to time-variant knowledge. 
    }
    \label{fig:CL}
\end{figure}

% To illustrate the issue, consider Figure~\ref{fig:CL}, which shows that LLMs often produce outdated or incorrect answers when queried about time-variant knowledge. While one might propose supplementing models like ChatGPT with an external, continually updated knowledge base, this approach still falls short in enabling real-time contextual understanding~\citep{mitchell2021fast, de2021editing}. Given these limitations, there is a pressing need for a framework that facilitates the real-time, internal updating of LLMs. Although recent studies have made initial strides in this direction~\citep{mitchell2021fast, de2021editing, zhu2020modifying, dhingra2022time, jang2021towards}, they have yet to comprehensively tackle the multifaceted challenges of rapid LLMs updating. 
As illustrated in Figure~\ref{fig:CL}, current LLMs often yield outdated or incorrect answers when confronted with time-sensitive questions. 
% This issue persists even when models like ChatGPT are supplemented with an external, constantly updated knowledge base~\citep{mitchell2021fast, de2021editing}. 
Addressing these constraints necessitates a framework that enables real-time, internal knowledge updating in LLMs. While some studies have begun addressing this need~\citep{mitchell2021fast, de2021editing, zhu2020modifying, dhingra2022time, jang2021towards}, they have not fully resolved the challenges associated with rapid LLM updating.

% We introduce a novel problem called \textit{Online Continual Knowledge Learning} (OCKL). Different from existing work in Continual Knowledge Learning (CKL)~\citep{jang2021towards}, OCKL prioritize the immediate, ongoing internal knowledge updating of models within significantly shorter timeframes, from days to hours or even seconds. This approach, unlike offline updating methods, ensures the model remains closely and synchronously attuned to the evolving global knowledge base. Subsequently, it necessities for single-pass updates (epoch$=$1) due to the high velocity and volume of incoming data \citep{aljundi2019gradient}. Such a setting has not been well studied for LM updates, and there is a lack of a robust benchmark for evaluation.
To tackle these issues, we propose the \textit{Online Continual Knowledge Learning} (OCKL) framework. OCKL differentiates itself from existing Continual Knowledge Learning (CKL) by prioritizing immediate, ongoing internal knowledge updates within significantly shorter timeframes, ranging from days to mere seconds. This approach, divergent from offline methods, requires single-pass updates (epoch$=$1) due to the high velocity and volume of incoming data~\citep{aljundi2019gradient}. OCKL presents a novel challenge in LM updates, for which a robust benchmark is essential yet currently absent.

% In this study, we develop a framework for dynamically updating the internal world knowledge of LMs through continual pre-training on high-velocity data streams. This approach specifically addresses the rapid pace and complexity inherent in real-world information streams. To evaluate model performance within this framework, we introduce two novel metrics: \textsc{Knowledge Acquisition Rate (KAR)} and \textsc{Knowledge Gap (KG)}. The KAR metric assesses the efficiency of text processing in tandem with the effectiveness of knowledge acquisition and retention, while the KG metric quantifies variances in learning during real-time data stream processing. These metrics are crucial for a comprehensive understanding of a model's adaptability to continuously evolving data. 
% In this study, we devise a framework for dynamically updating the internal world knowledge of LMs via continual pre-training on high-velocity data streams, addressing the challenges posed by real-world data. 
To evaluate LMs within our framework, we introduce two new metrics: \textsc{Knowledge Acquisition Rate (KAR)} and \textsc{Knowledge Gap (KG)}, assessing text processing efficiency, knowledge acquisition, retention, and real-time learning variances. Additionally, we examine the suitability of existing continual learning methods for OCKL, exploring model architectures and training methodologies that mitigate knowledge ``forgetting''~\citep{he2021analyzing, hu2021lora}. We also utilize advanced coreset selection techniques to enhance knowledge acquisition and reduce computational load~\citep{yoo2019learning, li2022camel}. This comprehensive approach establishes a robust baseline for the OCKL framework and lays the foundation for future research aimed at optimizing the adaptability and efficiency of LMs in real-time data environments.

% Furthermore, our investigation extends to examining the applicability of existing continual learning methods in OCKL. We explore various model architectures and training methodologies, particularly those shown to mitigate 'forgetting' during pre-training phases~\citep{he2021analyzing, hu2021lora}. In addition, we incorporate advanced coreset selection techniques, aiming to balance knowledge acquisition with computational efficiency~\citep{yoo2019learning, li2022camel}. This integrated approach not only sets a robust baseline for the OCKL framework but also lays the groundwork for future research endeavors focused on optimizing the efficiency and effectiveness of LMs in adapting to the dynamic nature of real-time data streams.

% In summary, the contributions of this paper are multifaceted and can be enumerated as follows:
\textbf{Contributions.} This paper presents multifaceted contributions:
% \begin{enumerate}
%     \item \textbf{Novel Framework and Benchmark}: We introduce \textbf{OCKL}, a novel framework for the Continual Learning of Language Models. 
%     \item \textbf{Baseline Approaches and Metrics}: To facilitate nuanced evaluation, we introduce innovative metrics, such as Knowledge Acquisition Rate and Knowledge Gap, which captures multiple dimensions of LMs' learning conditions.
%     \item \textbf{Empirical Observations and Challenges}: Our exhaustive analyses within the OCKL benchmark yield several key insights and challenges. Notably, rehearsal methods consistently outperform alternatives, albeit with a trade-off in buffer efficiency. 
% \end{enumerate}
\begin{enumerate}
    \item \textbf{Novel Framework and Benchmark}: The introduction of \textbf{OCKL}, a new framework designed to better understand the shortcomings of current LM updating practices facing high velocity data streams. 
    % evaluating the continual learning capability of LMs facing high velocity data streams.
    \item \textbf{Baseline Approaches and Metrics}: Innovative metrics like Knowledge Acquisition Rate and Knowledge Gap are introduced for nuanced evaluation of LMs' learning conditions.
    \item \textbf{Empirical Insights and Challenges}: Exhaustive analyses within the OCKL benchmark reveal crucial insights and challenges. For instance, rehearsal methods consistently outperform other approaches despite buffer inefficiencies.
\end{enumerate}

% real-time internal updating presents unique challenges, including: (1) the lack of a robust benchmark for evaluating both online knowledge acquisition and retention mechanisms; (2) the necessity for single-pass updates (epoch$=$1) due to the high velocity and volume of incoming data \citep{aljundi2019gradient}. 

% Particularly, OCKL differs from CKL by prioritizing the immediate, ongoing internal knowledge updating of models within significantly shorter timeframes, from days to hours or even seconds. This approach, unlike offline updating methods, ensures the model remains closely and synchronously attuned to the evolving global knowledge base.

% To address the challenges associated with updating LLMs with time-variant knowledge,

% This framework is designed to dynamically update the internal world knowledge of Language Models through continual pre-training on a high-velocity stream of current and relevant data. Our approach aims to fill the existing gaps in both models and methodologies, with a particular emphasis on accommodating the speed and complexity of real-world data streams. 

% Our work serves multiple objectives: it provides metrics for evaluating both the retention and acquisition of time-variant knowledge, and quantifies a model's alignment with real-world information post-training~\citep{yoo2019learning, li2022camel}. To further refine our framework, we introduce two novel metrics tailored to address the unique challenges posed by OCKL: 1)  \textsc{Knowledge Acquisition Rate (KAR):} This metric comprehensively assesses two attributes of various continual learning methods—namely, their text processing rate and their effectiveness in knowledge acquisition and retention.  2)  \textsc{Knowledge Gap (KG):} Designed to quantify variations in learning during real-time data stream processing. 

% Existing continual learning methods lay a foundation for evaluation, yet their applicability in the online experiments of online continual knowledge learning still requires determination. To address this, we explore model architectures and training methodologies that have shown promise in mitigating the phenomenon of ``forgettin'' during pre-training phases~\citep{he2021analyzing, hu2021lora}. Additionally, we capitalize on recent advancements in corset selection methods to improve knowledge acquisition performance while reducing computational overhead~\citep{yoo2019learning, li2022camel}. By integrating these methodologies, we establish a robust baseline for the OCKL framework, thereby laying the groundwork for future research focused on optimizing both the efficiency and effectiveness of knowledge updating in LMs. 



==> 5_Coreset_selection.tex <==
\section{Efficiency-Driven Coreset Selection in OCKL}
\label{sec:coreset}
Coreset selection is a strategy aimed at isolating a representative and informative subset from a comprehensive training dataset. The crux of its utility lies in enabling models to approximate the performance achieved when trained on the complete dataset. In the context of rehearsal-based continual learning, coreset selection has previously been employed as a mechanism to counteract catastrophic forgetting through the retention of a knowledge buffer~\cite {tiwari2022gcr, yoon2021online}. 

In this work, we extend the utility of coreset selection with a distinct focus on accelerating OCKL. By judiciously selecting pertinent data samples, our approach seeks not only to preserve antecedent knowledge but also to alleviate the computational demands inherent in the training process, thereby contributing to more efficient online learning systems. The ensuing discussion will explore three specific methods for coreset selection—Random Selection, K-Center Selection, and Model-Based Selection—each with its advantages and limitations in the context of OCKL. These methods are illustrated further in Appendix~\ref{coreset}.

\paragraph{Random Selection}
A straightforward method for reducing the size of the training data is random selection, which involves randomly choosing a subset of samples from the original dataset. This method's principal advantage is its simplicity and computational efficiency, as it obviates the need for complex selection criteria or domain-specific heuristics. This makes it especially suitable for scenarios involving large datasets where computational resources and time are limited.

Nonetheless, it is essential to acknowledge the limitations of random selection. Specifically, this method may inadvertently exclude informative or representative samples that could be crucial for model training. Moreover, it is ill-suited for applications involving imbalanced datasets since it does not take the distribution of the data into account.

\paragraph{K-Center Selection}
The K-Center problem, a classical issue in combinatorial optimization and graph theory, has recently been applied innovatively in active learning~\citep{sener2017active,borsos2020coresets}. In this approach, K centroids are identified to form a coreset, thereby enhancing the quality of the selected data. Extending this methodology, \citet{li2022camel} introduced the $\delta-cover$ concept to efficiently prune redundant data in image data streams. This innovation sets an upper bound on the objective function without the need for gradient or loss value computations, effectively reducing training overhead due to redundant or less-informative data instances.

However, transitioning this approach to text data and leveraging embeddings for coreset selection introduces several challenges that we addressed in this work. One such issue is the potential for loss of nuanced details during the embedding process, which can compromise the accuracy of K-center selection. Such an omission can result from the inadequacy of the embedding space in capturing the subtleties inherent in the original data. Another challenge lies in the distortion of inter-point distances within the original dataset when translated into the embedding space, thereby affecting the efficacy of greedy K-center algorithms. This could lead to selections that do not accurately represent the intrinsic structure of the original data.

\paragraph{Model-Based Selection}
Employing model states, such as loss and gradients, serves as a viable strategy for the selection of representative samples for training. Importance sampling techniques~\citep{johnson2018training, katharopoulos2018not, sinha2022experience} have shown promise in hastening the training process of deep neural models. Specifically, \citet{yoo2019learning} introduced small trainable modules within the model architecture to predict the loss values for untrained samples. These modules enable the subsequent utilization of samples with low predicted loss values for further training. Complementing this, \citet{yoon2021online} employed gradient analysis to gauge sample similarity, diversity, and affinity, allowing for the informed selection of data samples in each training iteration.

While these approaches potentially reduce the dataset size and expedite training, it is imperative to consider the computational costs associated with such techniques. Tasks like the training of auxiliary modules and the computation of data-affinity coefficients add an additional computational layer, which must be weighed against the benefits of the accelerated training process.


==> ICLR2024/2_Introduction.tex <==
\section{Introduction}
% 1, Introduce LLM need online continual learning
%         1) Why need continual learning （when new classes or tasks emerge, such models should acquire new knowledge on the fly, incorporating it with the current one.）
%         2) What is online continual learning 
%         3） Why need online continual learning (strong to online and low latency)


% Pre-training on extensive text corpora~\citep{petroni2019language} enables large language models (LLMs) like LLaMA~\citep{touvron2023llama} and GPT-3~\citep{brown2020language} to encapsulate a wide array of global knowledge within their parameters. Such attributes have proven advantageous for these models in excelling at Knowledge Intensive Language Tasks (KILT)\citep{petroni2021kilt}. The efficacy of these pre-trained language models has been further substantiated through evaluations conducted using the LAnguage Model Analysis (LAMA) task\citep{petroni2019language}, which serves as a method to assess world knowledge embedded in language models via slot-filling exercises without necessitating any preliminary fine-tuning. Furthermore, subsequent fine-tuning of these models on diverse KILT applications, including but not limited to question-answering and informed open dialogues, has yielded promising outcomes.

% While language models (LMs) are capable of storing extensive world knowledge, this information rapidly becomes outdated due to the fast-paced changes in global events. Although one could argue that an external, up-to-date knowledge base or vector database could be used in tandem with LMs to keep information current, this approach introduces latency in data retrieval and potentially weakens the model's ability to contextually interpret and integrate new information. Therefore, updating the internal structure of LMs themselves is a compelling necessity. 
% 1, define the problem OCKL

\begin{comment}
Large Language Models such as LLaMa2~\citep{touvron2023llama} and GPT-3~\citep{brown2020language}, pre-trained on extensive text corpora~\citep{petroni2019language}, have demonstrated significant prowess in Knowledge Intensive Language Tasks (KILT)~\citep{petroni2021kilt}. Their capabilities have been further validated through evaluations using the LAnguage Model Analysis (LAMA) task~\citep{petroni2019language}, which assesses the world knowledge encapsulated within these models. Despite their strengths, these models face challenges in adapting to the fast-paced changes in global events.
% , which forms the central issue this research aims to address.
While LLMs hold extensive reservoirs of world knowledge, such knowledge quickly becomes obsolete due to the dynamic nature of global events. Supplementing LLMs with an external, continually updated knowledge base or vector database might be a strategy, but this introduces latency and compromises the model's ability to integrate new data contextually~\citep{raffel2019exploring}.    
\end{comment}
Large Language Models (LLMs) such as LLaMa2~\citep{touvron2023llama} and GPT-3~\citep{brown2020language} have shown remarkable efficacy in Knowledge Intensive Language Tasks (KILT)~\citep{petroni2021kilt}. These models have been rigorously evaluated using the LAnguage Model Analysis (LAMA) framework~\citep{petroni2019language}, confirming their ability to encapsulate a wealth of world knowledge. However, they struggle to adapt to rapidly evolving global contexts. While one could consider augmenting LLMs with an external, continually updated knowledge base, this approach introduces latency and hampers the model's contextual understanding of new data~\citep{raffel2019exploring}.


\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{fig/CL-LMs.pdf}
    \caption{\small Static models such as T5~\citep{2020t5}, due to their knowledge cutoff, cannot provide timely answers to time-invariant knowledge. One solution is to use continuously trained language models.}
    \label{fig:CL}
\end{figure}

\begin{comment}
As a concrete example, as illustrated in Figure \ref{fig:CL}, when it comes to addressing questions related to time-invariant knowledge, the model often becomes outdated, resulting in erroneous responses.Supplementing ChatGPT with an external, updated database would not suffice, as the model would still face difficulties in real-time contextualization of this new information. In light of these complexities, the imperative for a framework that supports the continuous real-time internal updating of LLMs becomes evident. Recent studies have initiated preliminary explorations in this direction~\citep{mitchell2021fast, de2021editing, zhu2020modifying, dhingra2021time, jang2021towards}. However, these efforts have not yet coherently addressed the myriad challenges associated with rapid and effective updating of an LLM's internal knowledge base. Compared to closely related work in Continual Knowledge Learning (CKL)~\citep{jang2021towards}, the specific requirements for continuous real-time internal updating introduce three distinct challenges: (1) the absence of a robust benchmark that enables the systematic evaluation of both the knowledge updating and forgetting mechanisms in LLMs; (2) the need for single-pass updates (epoch$=$1) due to the sheer velocity and volume of incoming data; and (3) an as yet unmet requirement for extensive investigation into methodologies that allow for high-speed and accurate internal knowledge updates.    
\end{comment}
To illustrate the issue, consider Figure~\ref{fig:CL}, which shows that LLMs often produce outdated or incorrect answers when queried about time-variant knowledge. While one might propose supplementing models like ChatGPT with an external, continually updated database, this approach still falls short in enabling real-time contextual understanding~\citep{mitchell2021fast, de2021editing}. Given these limitations, there is a pressing need for a framework that facilitates the real-time, internal updating of LLMs. Although recent studies have made initial strides in this direction~\citep{mitchell2021fast, de2021editing, zhu2020modifying, dhingra2022time, jang2021towards}, they have yet to comprehensively tackle the multifaceted challenges of rapid LLM updating. Compared to existing work in Continual Knowledge Learning (CKL)~\citep{jang2021towards}, real-time internal updating presents unique challenges, including: (1) the lack of a robust benchmark for evaluating both online knowledge acquisition and retention mechanisms; (2) the necessity for single-pass updates (epoch$=$1) due to the high velocity and volume of incoming data \citep{aljundi2019gradient}.
% and (3) an unaddressed need for research into methods that enable swift and accurate internal knowledge updates.

\begin{comment}

Regarding the aforementioned challenges, this research presents a novel formulation for Continual Learning, termed \textit{Online Continual Knowledge Learning}. This framework emphasizes the dynamic renewal of internal world knowledge in LMs via continual pre-training on a high-velocity corpus stream enriched with new and up-to-date information. We aim to address the limitations and gaps in existing models and methodologies, particularly focusing on the rapidity and complexity of real-world data streams. To thoroughly evaluate the performance of LLMs under this framework, we contribute a specifically tailored benchmark, consisting of two parts: (1) \textit{Knowledge Stream}, which captures new data emergence and organizes them into coherent factual narratives; and (2) \textit{QA Stream}, which translates these narratives into a question-answer format. 
\end{comment}
To address the challenges associated with updating LLMs with time-variant knowledge, this study introduces a novel framework called \textit{Online Continual Knowledge Learning} (OCKL). This framework is designed to dynamically update the internal world knowledge of Language Models through continual pre-training on a high-velocity stream of current and relevant data. Our approach aims to fill the existing gaps in both models and methodologies, with a particular emphasis on accommodating the speed and complexity of real-world data streams. 
% To rigorously evaluate the efficacy of LLMs within this framework, we introduce a bespoke benchmark composed of two components: (1) \textit{Knowledge Stream}, designed to capture and organize emerging data into coherent factual narratives; and (2) \textit{QA Stream}, which converts these narratives into a question-answer format for evaluation.

\begin{comment}
The framework serves multiple purposes: it offers metrics for evaluating both the retention and acquisition of knowledge, while also quantifying the alignment of the model with real-world knowledge after each training cycle~\citep{yoo2019learning, li2022camel}. Further augmenting our framework, we introduce two innovative metrics to address unique challenges in OCKL: 1) \textsc{Learning Speed}—This metric holistically evaluates the dual attributes of various CL methods: their text processing rate and their efficacy in knowledge acquisition and retention. It furnishes a quantitative measure of a method's actual capability to assimilate and sustain knowledge in an OCKL setting. 2) \textsc{Knowledge Gap (KG)}—Formulated to measure variances in learning during real-time data stream processing, this metric serves as an incisive tool for quantifying both a model's knowledge absorption and its propensities for forgetting. It effectively gauges the disparity between a model's internalized knowledge and prevailing real-world information. 
\end{comment}
% Our framework serves multiple objectives: it provides metrics for evaluating both the retention and acquisition of time-variant knowledge, and quantifies a model's alignment with real-world information post-training~\citep{yoo2019learning, li2022camel}. To further refine our framework, we introduce two novel metrics tailored to address the unique challenges posed by OCKL: 1)  \textsc{Knowledge acquisition rate:} This metric comprehensively assesses the dual attributes of various Continual Learning (CL) methods—namely, their text processing rate and their effectiveness in knowledge acquisition and retention. It provides a quantitative measure of a method's actual capability to assimilate and sustain knowledge in an OCKL context. 2)  \textsc{Knowledge Gap (KG):} Designed to quantify variations in learning during real-time data stream processing, this metric serves as a precise tool for measuring both a model's capacity for knowledge absorption and its tendencies for forgetting. It effectively captures the disparity between a model's internalized knowledge and the current state of real-world information.

Our framework serves multiple objectives: it provides metrics for evaluating both the retention and acquisition of time-variant knowledge, and quantifies a model's alignment with real-world information post-training~\citep{yoo2019learning, li2022camel}. To further refine our framework, we introduce two novel metrics tailored to address the unique challenges posed by OCKL: 1)  \textsc{Knowledge Acquisition Rate (KAR):} This metric comprehensively assesses two attributes of various Continual Learning (CL) methods—namely, their text processing rate and their effectiveness in knowledge acquisition and retention.  2)  \textsc{Knowledge Gap (KG):} Designed to quantify variations in learning during real-time data stream processing. It effectively captures the disparity between a model's internalized knowledge and the current state of real-world information.

\begin{comment}
While existing CL methods offer a starting point for evaluation, our analysis reveals that the challenges unique to OCKL require specifically tailored approaches. To this end, we delve into model architectures and training methodologies~\citep{he2021analyzing, hu2021lora} that have demonstrated efficacy in mitigating the ``forgetting'' phenomenon during pretraining phases. Moreover, we leverage recent advancements in corset selection methods~\citep{yoo2019learning, li2022camel} to enhance knowledge acquisition performance while minimizing computational overhead. By synergistically combining these methodologies, we establish a robust baseline for the OCKL framework, setting the stage for future research aimed at optimizing both the efficiency and effectiveness of knowledge updating in LMs. In summary, the contributions of this paper are manifold and can be enumerated as follows:
\end{comment}
Existing continual learning methods lay a foundation for evaluation, yet their applicability in the online experiments of online continual knowledge learning still requires determination. To address this, we explore model architectures and training methodologies that have shown promise in mitigating the phenomenon of "forgetting" during pre-training phases~\citep{he2021analyzing, hu2021lora}. Additionally, we capitalize on recent advancements in corset selection methods to improve knowledge acquisition performance while reducing computational overhead~\citep{yoo2019learning, li2022camel}. By integrating these methodologies, we establish a robust baseline for the OCKL framework, thereby laying the groundwork for future research focused on optimizing both the efficiency and effectiveness of knowledge updating in LMs. In summary, the contributions of this paper are multifaceted and can be enumerated as follows:

\begin{comment}
\begin{enumerate}
\item We present \textit{Online Continual Knowledge Learning}, a novel formulation for Continual Learning of Language Models, and construct an accompanying benchmark that facilitates the rigorous assessment of both knowledge retention and acquisition in LMs. This benchmark operates on our newly created corpus specifically tailored for language modelling and infused with up-to-date world knowledge.

\item We engage in an in-depth exploration of existing LM architectures and training methodologies, establishing them as baseline approaches for the OCKL framework. To this end, we conduct extensive experiments on our OCKL benchmark, categorizing CL methods into regularization, rehearsal, and parameter-expansion approaches. We also integrate coreset selection techniques to optimize computational efficiency and knowledge acquisition efficacy. To enable a nuanced evaluation, we introduce novel metrics, such as \textsc{KG (\textbf{K}nowledge \textbf{G}ap)}, which encapsulates various facets of LMs' learning conditions.

\item Through comprehensive analyses carried out within the scope of the OCKL benchmark, we elucidate several pivotal observations and challenges. Notably, rehearsal methods consistently excel in comparison to alternative techniques, albeit at the expense of buffer efficiency. A significant finding is the detrimental impact of single-pass exposure to individual data points in inducing the 'forgetting' phenomenon. We further note that coreset selection methods have the capacity to substantially hasten training and alleviate forgetting, though these benefits come with inherent trade-offs in overall performance metrics. Crucially, we validate the applicability of OCKL setup across a variety of LM architectures, albeit with varying degrees of effectiveness in performance metrics.
\end{enumerate}
\end{comment}
% \begin{enumerate}
%     \item \textbf{Novel Framework and Benchmark}: We introduce Online Continual Knowledge Learning, a groundbreaking framework for the Continual Learning of Language Models (LMs). We also develop a corresponding benchmark that rigorously evaluates both knowledge retention and acquisition in LMs. This benchmark utilizes a newly curated corpus, specifically designed for language modeling and enriched with current world knowledge.

%     \item \textbf{Baseline Approaches and Metrics}: We undertake a comprehensive examination of existing LM architectures and training methodologies, establishing them as baseline approaches for the OCKL framework. Our extensive experiments on the OCKL benchmark categorize Continual Learning (CL) methods into three types: regularization, rehearsal, and parameter-expansion. We also incorporate coreset selection techniques to optimize both computational efficiency and knowledge acquisition. To facilitate nuanced evaluation, we introduce innovative metrics, such as Knowledge Gap (KG), which captures multiple dimensions of LMs' learning conditions.

%     \item \textbf{Empirical Observations and Challenges}: Our exhaustive analyses within the OCKL benchmark yield several key insights and challenges. Notably, rehearsal methods consistently outperform alternatives, albeit with a trade-off in buffer efficiency. We find that single-pass exposure to individual data points has a detrimental impact on knowledge retention, inducing the 'forgetting' phenomenon. Additionally, we observe that coreset selection methods can significantly accelerate training and mitigate forgetting, although these advantages come with inherent trade-offs in performance metrics. Importantly, we confirm the generalizability of the OCKL framework across various LM architectures, with differing levels of effectiveness in performance metrics.
% \end{enumerate}


\begin{enumerate}
    \item \textbf{Novel Framework and Benchmark}: We introduce Online Continual Knowledge Learning, a groundbreaking framework for the Continual Learning of Language Models. We also develop a corresponding benchmark that rigorously evaluates both knowledge retention and acquisition in LMs. 
    \item \textbf{Baseline Approaches and Metrics}: We undertake a comprehensive examination of existing LM architectures and training methodologies, establishing them as baseline approaches for the OCKL framework. To facilitate nuanced evaluation, we introduce innovative metrics, such as Knowledge Acquisition Rate and Knowledge Gap, which captures multiple dimensions of LMs' learning conditions.
    \item \textbf{Empirical Observations and Challenges}: Our exhaustive analyses within the OCKL benchmark yield several key insights and challenges. Notably, rehearsal methods consistently outperform alternatives, albeit with a trade-off in buffer efficiency. 
\end{enumerate}
% \begin{enumerate}
% \item We introduce the concept of \textit{Online Continual Knowledge Learning} for continual learning within Language Models and present a distinctive benchmark derived from a novel corpus that integrates time-invariant world knowledge.
    
% \item We conduct an in-depth analysis of current Language Model (LM) architectures, positing them as OCKL standards. Our research classifies Continual Learning (CL) strategies into three main categories: regularization, rehearsal, and parameter-expansion. We also utilize coreset selection to enhance efficiency and introduce metrics such as the Knowledge Gap and learning speed to evaluate the learning capabilities of LMs.

% \item Insights from our OCKL benchmark indicate that while rehearsal methods are superior, they require more memory buffer. Although coreset selection accelerates training and mitigates forgetting, it does come with certain performance compromises. 
% \end{enumerate}

% ============ rewrite according to Chunwei's suggestions =================
% Our thorough analysis leads us to a striking revelation: all evaluated CL methods, regardless of their theoretical effectiveness, underperform in a real-time setting. We trace this shortcoming to two main factors. First, the intrinsic online continual learning constrains the model from updating its knowledge in a single pass. This intrinsic constraint makes it challenging for models to effectively discern and prioritize meaningful knowledge.
% \cc{Second, the text stream data often suffers from quality issues when we utilize the property values of each entity as facts. This results in insufficient information, a lack of crucial details, and inconsistencies in the description of properties for the same entity.} This revelation highlights a crucial aspect of CL research that needs immediate attention. We need to devise strategies that not only facilitate efficient learning but are robust enough to manage and filter the relentless influx of data in real time. This is especially important when considering the need for LMs to adapt timely to the dynamic global knowledge landscape.

% In response to these challenges, we propose a special condition for online continual learning, i.e., data revisiting for each min-batch. Data would be learned more than one time by the model even in the single pass continual setting. Data revisiting enables LMs to extract and learn more discriminative knowledge to improve their performance despite the low quality of text streams in the online environment. However, data revisiting comes with the cost of learning speed for the same text stream, and reducing the data redundancy becomes necessary for our OCKL. Therefore, based on the data revisiting, we propose to leverage the core-set selection to choose representative samples for training. Compared with the single data revisiting process, core-set selection allows the model to focus on the novel and salient aspects of the data and thus achieves the trade-off between effective knowledge learning and training speed. Different core-set selection methods are applied in our online knowledge stream to enhance the practical utility of CL methods in continually updating LMs. Their results reveal that \cc{XXX}.

\begin{comment}
Large Language Models (LMs) such as LLaMA~\cite{touvron2023llama} and GPT-3~\cite{brown2020language} have demonstrated an impressive ability to embed a vast range of global knowledge within their parameters, owing to their pretraining phase on extensive, static text corpora~\cite{petroni2019language}. This has empowered these models to excel in Knowledge Intensive Language Tasks~\cite{petroni2021kilt}. However, a significant challenge lies in these models' inability to adapt to events occurring post their training phase, leading to a knowledge cutoff point and limiting their relevance in a dynamic world~\cite{jang2022continual}.
 
For instance, consider the event of Rishi Sunak assuming the role of the British Prime Minister. Language models trained before this occurrence typically underperform when tasked with queries about the prevailing political scenario in the UK, or any other task requiring knowledge of this recent development. To overcome these limitations and keep models up-to-date with dynamic world knowledge, a possible approach is to continually update these models with the latest factual knowledge. The proposed approach essentially transforms these models into dynamic entities capable of learning and adapting to real-time changes.

~\cite{jang2021towards} pioneered a novel avenue in continual learning (CL) research with the proposal of Continual Knowledge Learning (CKL). Their work explores the potential of LMs to learn and categorize knowledge into invariant, updated, and new groups, effectively providing a mechanism to evaluate how LMs manage a spectrum of knowledge types. One key finding highlighted in their research was the necessity of parameter expansion to reliably retain and learn knowledge simultaneously, acknowledging that CKL introduced unique challenges not addressed in traditional CL setups.
Furthering the concept of time-sensitive knowledge, ~\cite{dhingra2022time} introduced LMs as temporal knowledge bases, capable of integrating text with associated timestamps. Their work emphasized the challenges posed by factual knowledge with 'expiration dates' and proposed a diagnostic dataset for probing LMs for factual knowledge evolution over time. Notably, they proposed a simple technique to model text with its timestamp, which enhanced the memorization of seen facts and improved prediction calibration for unseen future facts.
~\cite{margatina2023dynamic} expanded this theme by exploring temporal concept drift, an evolving area that accounts for language and factual knowledge changes over time. Their study introduced a comprehensive framework capable of dynamically creating temporal test sets of various granularities from Wikidata. This approach allowed for a more holistic evaluation of how robustly an MLM can adapt over time and provided signals in case the model became outdated.

Despite the advances proposed by these studies, a common drawback persists—the assumption of virtually unlimited training time. This starkly contrasts with real-world scenarios, where data streams expose new data for prediction without waiting for the model's training completion. It emphasizes the need to transition towards real-time evaluations in the continual pretraining of LMs.

Building upon the principles established by Ghunaim et al.\cite{ghunaim2023real}, we extend their work to language models. Although their research focused on online continual learning in the context of computer vision, we adapt their emphasis on computational efficiency and real-time adaptability to meet the unique requirements of continual learning in language models. This allows us to bridge the theoretical and practical applications in NLP, in line with Ghunaim et al.'s commitment to practical continual learning.
However, this approach presents new challenges. With the high velocity and diversity of our data stream, our learning model must continuously adapt and incorporate new information. This continual learning process is complicated by the influx of data updates, which places strict constraints on the training time that can be devoted to learning from the incoming Wikidata stream. Traditional methods of continual learning, such as replay-based~\cite{aljundi2019gradient, yoon2021online, chrysakis2020online}, regularization~\cite{lopez2017gradient, chaudhry2018efficient}, and parameter isolation methods~\cite{rusu2016progressive, hu2018overcoming}, can slow down the entire learning process due to their significant computational time, especially when dealing with large real-time data streams.

To address the challenges of training language models with continually updated information, we propose a unique online continual learning benchmark specifically designed for LM pretraining. We construct our dataset using Wikipedia's ever-evolving knowledge, mirroring global knowledge transformation. This dataset, referred to as the \textbf{knowledge stream}, facilitates the model's factual learning. Simultaneously, we use a corresponding question-answer (QA) data pair, or the \textbf{QA stream}, to provide real-time performance assessments.
In our benchmarking exercise, we evaluate models not only in terms of accuracy (ACC) and backward transfer (BWT) but also in terms of latency. Furthermore, we, for the first time, propose to leverage DTW (dynamic time warping) to quantify the relative distance between the actual knowledge growth curve and the model's knowledge growth curve. We assess various prevalent CL techniques including lora~\cite{hu2021lora}, Kadapter~\cite{wang2020k}, etc.

Our comprehensive analysis leads us to a striking revelation: regardless of their theoretical effectiveness, all evaluated Continual Learning (CL) methods are found wanting in a real-time setting. We attribute this shortcoming to two major factors. Firstly, the incoming data stream's redundancy puts a significant strain on the learning system, making it difficult for the models to discern and prioritize new knowledge effectively. Secondly, the text stream data's quality often falls short of the mark, providing inadequate or even misleading information for learning. This revelation casts a spotlight on an important aspect of CL research that needs immediate addressing. There is a clear necessity to devise strategies that not only enable efficient learning but also are robust enough to manage and filter the relentless influx of data in real-time. This becomes even more crucial when we consider the importance of LMs' timely adaptability to the dynamic global knowledge landscape.

In light of these challenges, our work introduces a data distillation method, a promising step towards alleviating these issues. We envision this method as a means to strike an optimal balance between model performance and training latency. By distilling the incoming data, we aim to trim the redundancy that has been plaguing the training process. This streamlined approach allows the model to focus on the salient and novel aspects of the data, thus enhancing the overall efficiency of the learning process. Our initial findings are heartening. The data distillation method, when tested, demonstrates promising improvements. It not only ameliorates training latency but also ensures no compromise on model performance. Although the method is still in its nascent stages, the positive trends in our results indicate its potential to significantly enhance the practical utility of CL methods in continually updating LMs. We will delve into our findings in the ensuing sections, revealing that XXX.

\textbf{Contributions.} We summarize our conclusions as follows: 
\begin{enumerate}
    \item{}  
    \item{}
    \item{}
\end{enumerate}
\end{comment}

% In the past, research on language models (LM) for continuous learning has garnered attention. \cite{jin2022lifelong} proposed continuous learning on a corpus encompassing diverse domains, addressing the issue of forgetting via knowledge distillation. Similarly, \cite{qin-etal-2022-elle} circumvented forgetting by incorporating prompts during the pre-training phase. Despite their efforts, these studies remain challenged by changes in knowledge across varying domains. \cite{fisch2023robust} conducted a more targeted exploration, investigating efficient continuous learning of LM under task-incremental conditions. Concurrently, \citep{dhingra-etal-2022-time} have viewed LMs as temporal knowledge bases, developing models that integrate text with its corresponding timestamps. \citep{jang2022continual}, whose work is most similar to ours, contributed a valuable dataset for evaluating the model's capacity for both updating and forgetting. Unfortunately, the aforementioned studies are predominantly grounded in the offline continual learning paradigm, they operate under the presumption of near-infinite time and computational resources, alongside the availability of datasets with distinct task boundaries. To that end, there has recently been a growing interest in the more realistic setting – Online Continual Learning (OCL).  However, it is regrettable that the prevailing benchmarks for assessing the continual learning capacity of language models are not robust enough to tackle the demanding challenges of high throughput and relatively fast responses inherent in an online environment.



% 3， OCLStream: our task setting and summary challenge 
%             1) Real-time inference: do not require task identifiers at inference time; 
%             2) Efficient: have a bounded memory and computing throughout the entire training phase.
%             3) Challenge:
%                 1) Stream redundancy and complexity
%                 2）Limited computational resources and the need for real-time reasoning
%                 3）Catastrophic forgetting

% In consideration of the recent advancements by Ghunaim et al.\cite{ghunaim2023real} in the area of online continual learning (OCL), we've identified two main challenges when applying real-time evaluation to Language Models (LMs). First, we lack comprehensive datasets that span a broad spectrum of time granularities. Second, it's challenging to efficiently integrate and manage the myriad of CL components frequently used in research.

% The insufficiency of the existing text datasets becomes evident when we attempt to dynamically evaluate how LMs acquire and assimilate knowledge across various time granularities. The limited nature of these datasets introduces a level of uncertainty, raising questions about whether an LM can effectively retain outdated knowledge and incorporate new information.

% Our second challenge is rooted in the training and testing methodology commonly used for LMs. Traditionally, LMs are pretrained on a static text corpus, and their performance is evaluated using corresponding query-answer data pairs. However, this traditional approach might not suit all real-world applications where there is a need for the model to adapt in real-time. This discrepancy, a challenge that is not as prevalent in many other machine learning domains, can lead to performance degradation when these models are used in dynamic, real-time settings.

% To address these challenges, we propose a unique online continual learning benchmark, specifically designed for LM pretraining. We construct our dataset \dataset using Wikipedia's ever-evolving knowledge, effectively mirroring global knowledge transformation. This dataset, known as the \textbf{knowledge stream}, is used to facilitate the model's factual learning. Simultaneously, a corresponding question-answer (QA) data pair, referred to as the \textbf{QA stream}, is used to provide real-time performance assessments.

% Our work extends the principles laid out by Ghunaim et al.\cite{ghunaim2023real} to the realm of language models. While Ghunaim et al. focused on online continual learning in the context of computer vision, our approach repurposes their focus on computational efficiency and real-time adaptability for the unique requirements of continual learning in language models. This method allows us to bridge the gap between theoretical considerations and practical application in NLP, echoing Ghunaim et al.'s commitment to practical continual learning.

% The potential of online continuous learning (OCL) for absorbing factual knowledge is considerable, particularly evidenced by environments such as Twitter, where about 350K tweets are posted every minute on various trending topics~\cite{sayce_2022}. This high-velocity data stream contains a vast diversity of factual knowledge, such as news reports, necessitating that the learning model adapts continuously to incorporate new information. Given the massive rate of data updates, there is a critical constraint on the training time that can be allotted to learning from incoming tweets. This constraint is a significant challenge often underemphasized in previous OCL literature.  In response to this, we propose in this paper a real-time evaluation benchmark for OCL for LMs that takes into account \red{training computational complexity, specifically efficiency, and latency.}


% 4,  our method: sample data selection
%           1) Summary of our method
%           2) Describe our approach （？）
%              1， define the state of stream data
%              2,  stateful data selection
%              3,  stateful data replay
% 5, our contribution

% Owing to the high-velocity and diversity of factual knowledge within our data stream, it's imperative for our learning model to continuously adapt and incorporate new information. However, given the massive influx of data updates, we encounter a strict constraint on the training time that can be devoted to learning from the incoming Wikidata stream. Traditional continual learning has harnessed three primary categories of methods to mitigate forgetting, including replay-based~\cite{aljundi2019gradient, yoon2021online, chrysakis2020online}, regularization~\cite{lopez2017gradient, chaudhry2018efficient}, and parameter isolation methods~\cite{rusu2016progressive, hu2018overcoming}. Nevertheless, these methods incur significant computational time, which could detrimentally slow the entire learning process, especially during the handling of voluminous real-time data streams.

% To address this challenge, we propose a simple yet effective data distillation method aimed at achieving a balance between performance and training latency. This approach serves to minimize the impact of redundant data on training time. In our benchmarking exercise, we evaluate models on multiple fronts: accuracy (ACC), backward transfer (BWT), and latency. Moreover, we introduce a novel evaluation metric: OCL-DTW (online continual learning dynamic time warping), designed to quantify the relative distance between the actual knowledge growth curve and the model's knowledge growth curve.

% After establishing our baseline, we assess a selection of prevalent incremental learning techniques. Our findings, which we will delve into in the ensuing sections, reveal that XXX.

% In this study, we construct our dataset by utilizing Wikipedia, harnessing the evolving knowledge and its changes within the platform as a representation of the world's knowledge transformation. This serves as a knowledge data stream, facilitating the model's learning of factual information. Concurrently, we construct a question-answer (QA) data stream through a similar process for real-time assessment. 


